Beyond Tracking: Selecting Memory and Refining Poses for Deep Visual Odometry

Most previous learning-based visual odometry (VO) methods take VO as a pure tracking problem. In contrast, we present a VO framework by incorporating two additional components called Memory and Refining. The Memory component preserves global information by employing an adaptive and efficient selection strategy. The Refining component ameliorates previous results with the contexts stored in the Memory by adopting a spatial-temporal attention mechanism for feature distilling. Experiments on the KITTI and TUM-RGBD benchmark datasets demonstrate that our method outperforms state-of-the-art learning-based methods by a large margin and produces competitive results against classic monocular VO approaches. Especially, our model achieves outstanding performance in challenging scenarios such as texture-less regions and abrupt motions, where classic VO algorithms tend to fail.

==> README <==
This package enables you to embed Python code (www.python.org) in LaTeX and insert the output into your LaTeX document.

In you LaTeX document insert:

\usepackage{python}
...
\begin{python}[optional.py]
print("42")
\end{python}

The file optional.py is included together with the code between \begin{python} and \end{python}. Hence, you can extract common code to a shared file.

Compile the document with the shell escape option and of course Python installed:

% latex -shell-escape document.tex

or insert/change "shell_escape = t" in your texmf.cnf

If you have any comments, suggestions, or patches please email them to me.

Please note that this material is subject to the GNU General Public License as published by the Free Software Foundation; either version 2 of the License, or (at your option) any later version.
See http://www.gnu.org/copyleft/gpl.html for the details of that license.

Martin R. Ehmsen
martin@ehmsen.org

==> SupplySections/Generalization.tex <==
\section{Generalization}
\label{sec:generalization}

%\input{fig_table/fig_kitti_extra}

We tentatively test the generalization ability of our model on the Seq 11-12 of the KITTI dataset \cite{geiger2012kitti} against state-of-the-art monocular methods include GFS-VO \cite{xue2018fea}, VISO2-M \cite{geiger2011stereoscan} and ORB-SLAM2 \cite{mur2017orb-slam2} (with loop closure disabled). Since there are no ground-truth supplied for these sequences, similar with GFS-VO, we utilize the results of stereo VISO2 (VISO2-S) \cite{geiger2011stereoscan} as references.
This time, our model is trained the Seq 00-10 as GFS-VO \cite{xue2018fea} to avoid over-fitting and maximize the ability of generalization. 

Qualitative comparison is illustrated in Figure~\ref{fig:trajectory_kitti_extra}. VISO2-M \cite{geiger2011stereoscan} suffers from severe error accumulation, because it is a classic tracking VO by integrating frame-wise poses as the entire trajectories. ORB-SLAM2 \cite{mur2017orb-slam2} partially alleviates the problem with a global map to assist tracking. Although achieving promising performance in regular environments (Seq 11, 15), it bears large scale drift in complicated scenes (Seq 13, 14, 16, 18, 19). The requirement of sophisticate map initialization degrades its ability to handle situations with high speeds (Seq 12, 17).

%In contrast, owing to the introduced the \textit{Memory} component for global information gathering and the \textit{Refining} component for ameliorating previous outputs, our model barely suffers from scale drift than GFS-VO \cite{xue2018fea} and VISO2-M \cite{geiger2011stereoscan}. Our model produces very close results with ORB-SLAM2 \cite{mur2017orb-slam2} in regular scenes. While in complicated environments (Seq 13, 16, 18, 19), our model achieves better performance. Note that our system works well even in challenging conditions including high speeds (Seq 12, 17) where ORB-SLAM2 fails.

\begin{figure*}[htbp]
	\begin{center}
		%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
		\includegraphics[width=1\linewidth]{result_images/extra_orbm_visom/crop/kitti_frames}
	\end{center}
	\caption{Trajectories of our model trained with sequences consisting of different frames on the TUM-RGBD dataset \cite{tum12iros} (from left to right: fr3/nstr\_tex\_near\_loop, fr2/pioneer\_360, fr3/str\_ntex\_far, fr3/nstr\_ntex\_near\_loop, fr3/str\_tex\_far, fr3/large\_cabinet).}
	\label{fig:trajectory_kitti_frames}
\end{figure*}
 


==> SupplySections/Influence.tex <==
\section{The Influence of Sequence Length}
\label{sec:sequence_length}
In this section, we test the influence of sequence length on the results of our proposal. Theoretically, the better performance can be achieved when given more frames. We compare the results with sequences constructing of 5, 7, 9, and 11 frames on the KITTI \cite{geiger2012kitti} (see Table~\ref{tab:table_kitti_00_10_frames}) and TUM-RGBD dataset (see Table~\ref{table:tum_frames_full}) \cite{tum12iros} respectively.

As we can see from Table~\ref{tab:table_kitti_00_10_frames} and \ref{table:tum_frames_full}, the results of our model are improved by introducing more frames. Since our model remembers information over the whole sequence and refines previous outputs, the performance is intuitively improved by giving more observations. Figure~\ref{fig:trajectory_kitti_frames} and \ref{fig:trajectory_tum_frames} illustrate the qualitative comparison.

\input{fig_table/table_kitti_00_10_frames}
\input{fig_table/fig_kitti_frames}

\input{fig_table/table_tum_frames_full}
\input{fig_table/fig_tum_frames}

%\input{fig_table/table_tum_frames_tracking}

\clearpage


==> SupplySections/Introduction.tex <==
\section{Introduction}
In the supplementary material, we supply additional technical details and results for our paper. In Sec.\ref{sec:generalization}, we test the generalization ability of our network on the extra sequences of the KITTI benchmark \cite{geiger2012kitti}. We also give the details of training and test sequences used in the TUM-RGBD dataset \cite{tum12iros}.

\section{Training Data in the TUM-RGBD dataset}
\label{sec:training_data_tum}
We select 19 sequences as training data (see Table~\ref{table:tum_training}) and 10 sequences for testing (see Table~\ref{table:tum_testing}). Both the training and testing sequences include various conditions such as regular environments with rich textures, textureless scenes with obvious structures, or sequences recorded with abrupt motions. This dataset was collected by handheld cameras at up to 30 fps, resulting in much overlapped between consecutive frames, which hampers the generalization ability of the model. To cope with problem, we randomly select 16578 short sequences for training, yet overlapped frames are reduced. While for testing sequences, the pose of each frame is recovered

\input{fig_table/table_tum_training}
\input{fig_table/table_tum_testing}

%\clearpage

==> fig_table/fig_attention.tex <==
\begin{figure}[t]
	\centering
	\subfigure[SRNN]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.cm]{result_images/srnn/crops/kitti_05}
			\label{fig:kitti10_a}
	\end{minipage}}
	\vspace{-0.3cm}
	%\hspace{1cm}
	%\qquad
	\subfigure[SRNN\_se]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.cm]{result_images/srnn_se/crops/kitti_05}
			\label{fig:kitti10_b}
	\end{minipage}}
	\subfigure[SRNN\_point]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.cm]{result_images/srnn_point/crops/kitti_05}
			\label{fig:kitti10_c}
	\end{minipage}}
	%\qquad
	\subfigure[SRNN\_channel]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.cm]{result_images/srnn_channel/crops/kitti_05}
			\label{fig:kitti10_d}
	\end{minipage}}
	\caption{Qualitative comparison of the trajectories of the vanilla and three guided models for separate motion estimation on the KITTI Seq 10.}
	\label{fig:variation_kitti10}
\end{figure}
\setlength{\tabcolsep}{1.4pt}


==> fig_table/fig_error_each_view.tex <==
\begin{figure}[t]
	\centering
	\subfigure[Rotational error of each view]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.2cm]{result_images/attention/rot_mean_view}
			\label{fig:variations_rotation}
	\end{minipage}}
	\subfigure[Translational error of each view]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.2cm]{result_images/attention/trans_mean_view}
			\label{fig:variations_translation}			
	\end{minipage}}
	\caption{Rotational (a) and translational (b) errors along each view of the network for joint motion prediction, vanilla and guided models for separate pose recovery.}
	\label{fig:result_attention}
\end{figure}
\setlength{\tabcolsep}{1.4pt}

==> fig_table/fig_kitti_00_10.tex <==
\begin{figure*}[t]
	%\setlength{\abovecaptionskip}{-1cm}
	%\setlength{\belowcaptionskip}{-1cm}
	\centering
	\subfigure[Seq 03]{
		\begin{minipage}{0.32\textwidth}
			\centering
			\includegraphics[height=4.cm]{result_images/orbm/crop/kitti_03}
			\label{fig:trajectory_kitti_00_03}
	\end{minipage}}
	\subfigure[Seq 04]{
	\begin{minipage}{0.32\textwidth}
		\centering
		\includegraphics[height=4.cm]{result_images/orbm/crop/kitti_04}
		\label{fig:trajectory_kitti_00_04}
	\end{minipage}}
	\subfigure[Seq 05]{
		\begin{minipage}{0.32\textwidth}
			\centering
			\includegraphics[height=4.cm]{result_images/orbm/crop/kitti_05}
			\label{fig:trajectory_kitti_00_05}
	\end{minipage}}
	\subfigure[Seq 06]{
	%\setlength{\abovecaptionskip}{-1cm}
	\begin{minipage}{0.32\textwidth}
		\centering
		\includegraphics[height=4.cm]{result_images/orbm/crop/kitti_06}
		\label{fig:trajectory_kitti_00_06}
	\end{minipage}}
	\subfigure[Seq 07]{
		%\setlength{\abovecaptionskip}{-1cm}
		\begin{minipage}{0.32\textwidth}
			\centering
			\includegraphics[height=4.cm]{result_images/orbm/crop/kitti_07}
			\label{fig:trajectory_kitti_00_07}
	\end{minipage}}
	\subfigure[Seq 10]{
	\begin{minipage}{0.32\textwidth}
		\centering
		\includegraphics[height=4.cm]{result_images/orbm/crop/kitti_10}
		\label{fig:trajectory_kitti_00_10_10}
	\end{minipage}}

	\caption{The trajectories of ground-truth, SfmLearner \cite{zhou2017egomotion}, Depth-VO-Feat \cite{zhan2018feature}, GFS-VO \cite{xue2018fea} and our model on Seq 03, 04, 05, 06, 07 and 10 of the KITTI benchmark. GFS-VO \cite{xue2018fea} and our model are trained on the Seq 00, 02, 08, and 09 supervisely, while SfmLearner \cite{zhou2017egomotion} and Depth-VO-Feat \cite{zhan2018feature} are trained on Seq 00-08 in an unsupervised manner. }
	\label{fig:trajectory_kitti_00_10}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_table/fig_kitti_00_10_4.tex <==
\begin{figure}[t]
	%\setlength{\abovecaptionskip}{-1cm}
	%\setlength{\belowcaptionskip}{-1cm}
	\centering
	\subfigure[Seq 03]{
		\begin{minipage}{0.23\textwidth}
			\centering
			\includegraphics[height=3.cm]{result_images/orbm/crop/kitti_03}
			\label{fig:trajectory_kitti_00_03}
	\end{minipage}}
	\subfigure[Seq 05]{
		\begin{minipage}{0.23\textwidth}
			\centering
			\includegraphics[height=3.cm]{result_images/orbm/crop/kitti_05}
			\label{fig:trajectory_kitti_00_05}
	\end{minipage}}
	\subfigure[Seq 07]{
		%\setlength{\abovecaptionskip}{-1cm}
		\begin{minipage}{0.23\textwidth}
			\centering
			\includegraphics[height=3.cm]{result_images/orbm/crop/kitti_07}
			\label{fig:trajectory_kitti_00_07}
	\end{minipage}}
	\subfigure[Seq 10]{
	\begin{minipage}{0.23\textwidth}
		\centering
		\includegraphics[height=3.cm]{result_images/orbm/crop/kitti_10}
		\label{fig:trajectory_kitti_00_10_10}
	\end{minipage}}

	\caption{The trajectories of ground-truth,  Depth-VO-Feat \cite{zhan2018feature}, GFS-VO \cite{xue2018fea}, ORB-SLAM2 \cite{mur2017orb-slam2} and our model on Seq 03, 05, 07 and 10 of the KITTI benchmark. GFS-VO \cite{xue2018fea} and our model are trained on the Seq 00, 02, 08, and 09 supervisely, while Depth-VO-Feat \cite{zhan2018feature} is trained on Seq 00-08 in an unsupervised manner.}
	\label{fig:trajectory_kitti_00_10}
\end{figure}
\setlength{\tabcolsep}{1.4pt}


==> fig_table/fig_kitti_11_21.tex <==
\begin{figure}[t]
	\centering
	\subfigure[Seq 11]{
		\begin{minipage}{0.3\textwidth}
			\centering
			\includegraphics[height=2.7cm]{result_images/extra/orbs/noorb/kitti_11}
	\end{minipage}}
	\vspace{-0.4cm}
	\subfigure[Seq 12]{
		\begin{minipage}{0.3\textwidth}
			\centering
			\includegraphics[height=2.7cm]{result_images/extra/orbs/noorb/kitti_12}
	\end{minipage}}
	\subfigure[Seq 13]{
		\begin{minipage}{0.3\textwidth}
			\centering
			\includegraphics[height=2.7cm]{result_images/extra/orbs/noorb/kitti_13}
	\end{minipage}}
	\subfigure[Seq 14]{
		\begin{minipage}{0.3\textwidth}
			\centering
			\includegraphics[height=2.7cm]{result_images/extra/orbs/noorb/kitti_14}
	\end{minipage}}
	\vspace{-0.4cm}
	\subfigure[Seq 15]{
		\begin{minipage}{0.3\textwidth}
			\centering
			\includegraphics[height=2.7cm]{result_images/extra/orbs/noorb/kitti_15}
	\end{minipage}}
	\subfigure[Seq 16]{
		\begin{minipage}{0.3\textwidth}
			\centering
			\includegraphics[height=2.7cm]{result_images/extra/orbs/noorb/kitti_16}
	\end{minipage}}
	\subfigure[Seq 18]{
		\begin{minipage}{0.3\textwidth}
			\centering
			\includegraphics[height=2.7cm]{result_images/extra/orbs/noorb/kitti_18}
	\end{minipage}}
	\subfigure[Seq 19]{
		\begin{minipage}{0.3\textwidth}
			\centering
			\includegraphics[height=2.7cm]{result_images/extra/orbs/noorb/kitti_19}
	\end{minipage}}
	\subfigure[Seq 20]{
		\begin{minipage}{0.3\textwidth}
			\centering
			\includegraphics[height=2.7cm]{result_images/extra/orbs/noorb/kitti_20}
	\end{minipage}}
	%\vspace{-0.3cm}
	\caption{The predicted trajectories on KITTI sequences 11-20. Results of VISO2-S are used as reference since ground-truth poses of these sequences are unavailable.}
	\label{fig:trajectory_kitti_11-21}
	%\vspace{0.cm}
\end{figure}
\setlength{\tabcolsep}{1.4pt}

==> fig_table/table_icl_rpe.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
%\setlength{\tabcolsep}{2.0pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table}[b]
	%\scriptsize
	\centering
		\caption{Evaluation on the ICL\_NUIM dataset. Results of DRFE, DEMO, DVO and MWO are taken directly from \cite{kim2017visual}.}
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{c|cccccc}
				\hline
				\hline
				Sequence & $\mathbf{SRNN\_channel}$ & $\mathbf{SRNN}$ & DFRE \cite{kim2017visual}& DEMO \cite{demo2014zhang} & DVO \cite{dvo2013robust} & MWO \cite{mwo2016zhou}   \\
				\hline
				lr kt1 & $\mathbf{0.009}$ & 0.010 & 0.021 & 0.020 & 0.023 & 0.100  \\
				lr kt2 & $\mathbf{0.019}$ & 0.019  & 0.031 & 0.090 & 0.084 & 0.052 \\
				\hline
				of kt1 & $\mathbf{0.011}$ & 0.015 & 0.014 & 0.054 & 0.045 & 0.263  \\
				of kt2 & 0.019 & 0.021 & $\mathbf{0.015}$ & 0.079 & 0.065 & 0.047 \\ 
				\hline
				\hline
			\end{tabular}	
		\end{center}
		%\end{left}
	%\end{threeparttable}}
	% Relative pose errors of four algorithms (from \cite{kim2017visual}) and our method on ICL\_NUIM dataset.
	%The four compared algorithms use depth information, while our method utilizes monocular RGB images only.
	%Predicted trajectories of ORB\_SLAM \cite{mur2017orb-slam2} are aligned with ground-truth due to unknown scale. VISO2\_M \cite{geiger2011stereoscan} recovers scale using the fixed camera height as priori.}
	\label{table:icl}
\end{table}
\setlength{\tabcolsep}{1.4pt}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{2cm}

==> fig_table/table_kitti.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
\setlength{\tabcolsep}{2.4pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table}[t]
	\scriptsize
	\centering
		\caption{Results on the KITTI dataset. DeepVO \cite{wang2017deepvo} and our models are trained on Seq 00, 02, 08 and 09, while ESP-VO \cite{wang2017espvo} uses extra Seq 01 in training sets.}
	%\begin{threeparttable}
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{lclclclclclcl}
				\hline
				\hline
				& \multicolumn{12}{c}{Sequence} \\
				% \cline{2-15} 
				Method & \multicolumn{2}{c}{03} & \multicolumn{2}{c}{04} & \multicolumn{2}{c}{05} & \multicolumn{2}{c}{06} & \multicolumn{2}{c}{07} & \multicolumn{2}{c}{10} \\ 
				%Method & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} &  \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} \\
				& $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$    \\
				\hline
				% DeepVO &  \multicolumn{2}{c} {$- \quad -$} &  \multicolumn{2}{c}{$8.49 \quad 6.89$} &  \multicolumn{2}{c}{$7.19 \quad 6.97$} &  \multicolumn{2}{c}{$2.62 \quad 3.61$} &  \multicolumn{2}{c}{$5.42 \quad 5.82$} &  \multicolumn{2}{c}{$3.91 \quad 4.60$} &  \multicolumn{2}{c}{$8.11 \quad 8.83$} \\
				%ORB\_SLAM-S [5] & 0.71 & 0.18 & 0.48 & 0.13 & 0.40 & 0.16 & 0.51 & 0.15 & 0.50 & 0.28 & 0.60 & 0.27 \\
				%ORB\_SLAM \cite{mur2017orb-slam2} & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				%ORB\_SLAM-M [5] & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				VISO2-S \cite{geiger2011stereoscan} & 3.21 & 3.25 & 2.12 & 2.12 & 1.53 & 1.60 & 1.48 & 1.58 & 1.85 & 1.91 & 1.17 & 1.30 \\
				\hline
				VISO2-M \cite{geiger2011stereoscan}   & 8.47 & 8.82 & 4.69 & 4.49 & 19.22 & 17.58 & 7.30 & 6.14 & 23.61 & 19.11 & 41.56 & 32.99 \\
				%ORB\_SLAM \cite{mur2015orb1} & 21.07 & 18.36 & 4.46 & 5.60 & 26.01 & 34.27 & 17.47 & 17.17 & 24.53 & 38.90 & 86.51 & 98.90 \\
				\hline
				\hline
			\end{tabular}
			\label{result_kitti}
			
			%\begin{left}
			\begin{tablenotes}
				%\left
				%\item $*$ORB\_SLAM \cite{mur2017orb-slam2} is not evaluated with other methods since it results are aligned with ground-truth using 7-DoF (rigid body + scale) transformation.
				\footnotesize
				\item $t_{rel}: $ average translational RMSE drift (\%) on length from 100, 200 to 800 m.
				\item $r_{rel}: $ average rotational RMSE drift (${}^{\circ}$/100m) on length from 100, 200 to 800 m.
				%\item Our models and DeepVO are trained on Sequence 00, 02, 08, and 09, while ESP-VO uses additional Sequence 01 for training.
			\end{tablenotes}
		\end{center}
		%\end{left}
	%\end{threeparttable}}
% The best results of monocular VO are highlighted.} %Predicted trajectories of ORB\_SLAM \cite{mur2017orb-slam2} are aligned with ground-truth due to unknown scale. VISO2\_M \cite{geiger2011stereoscan} recovers scale using the fixed camera height as priori.}
	\label{table:table_kitti}
\end{table}
\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}

==> fig_table/table_kitti_00_10_classic_visom.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
%\setlength{\tabcolsep}{3.pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table}[t]
	%\scriptsize
	\small
	\centering
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{ccccccccc}
				\hline
				\hline
				& \multicolumn{8}{c}{Method} \\
				% \cline{2-15} 
				Seq & \multicolumn{2}{c}{Ours} & \multicolumn{2}{c}{ORB-SLAM2} & \multicolumn{2}{c}{ORB-SLAM2} & \multicolumn{2}{c}{VISO2-M} \\ 
				%Method & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} &  \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} \\
				& $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$  \\
				\hline
				% DeepVO &  \multicolumn{2}{c} {$- \quad -$} &  \multicolumn{2}{c}{$8.49 \quad 6.89$} &  \multicolumn{2}{c}{$7.19 \quad 6.97$} &  \multicolumn{2}{c}{$2.62 \quad 3.61$} &  \multicolumn{2}{c}{$5.42 \quad 5.82$} &  \multicolumn{2}{c}{$3.91 \quad 4.60$} &  \multicolumn{2}{c}{$8.11 \quad 8.83$} \\
				%ORB\_SLAM-S [5] & 0.71 & 0.18 & 0.48 & 0.13 & 0.40 & 0.16 & 0.51 & 0.15 & 0.50 & 0.28 & 0.60 & 0.27 \\
				%ORB\_SLAM \cite{mur2017orb-slam2} & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				%ORB\_SLAM-M [5] & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				%VISO2-S \cite{geiger2011stereoscan} & 3.21 & 3.25 & 2.12 & 2.12 & 1.53 & 1.60 & 1.48 & 1.58 & 1.85 & 1.91 & 1.17 & 1.30 \\
				03 & 3.32 & 2.10 & 0.93 & 0.20 &  8.47 & 8.82  \\
				04 & 2.96 & 1.76 & 0.88 & 0.21 & 4.69 & 4.49 \\
				05 & 2.59 & 1.25 & 12.05 & 0.2 & 19.22 & 17.58  \\
				06 & 4.93 & 1.90&  19.59 & 0.23 & 7.30 & 6.14  \\
				07 & 3.07 & 1.76 &  13.63 & 0.37 & 23.61 & 19.11 \\
				10 & 3.94 & 1.72 &  3.68 & 0.48 & 41.56 & 32.99 \\
				Avg & 3.47 & 1.75 &  24.97 & 0.30 & 17.48 & 16.52 \\
				%VISO2-M \cite{geiger2011stereoscan}   & 8.47 & 8.82 & 4.69 & 4.49 & 19.22 & 17.58 & 7.30 & 6.14 & 23.61 & 19.11 & 41.56 & 32.99 \\
				%\hline
				%\textbf{RNN\_g} & 11.10 & 6.28 & 11.37 & 3.89 & 9.97 & 3.81 & 24.39 & 9.64 & 15.39 & 4.18 & 15.37 & 6.92 \\
				%$\mathbf{RNN}$ & 6.36 & 3.62 & 5.95 & 2.36 & 5.85 & 2.55 & 14.58 & 4.98 & 5.88 & 2.64 & 7.44 & 3.19 & 5.96 & 6.12\\
				
				%$\mathbf{Ours}$  & $\mathbf{3.32}$ & $\mathbf{2.10}$ & 2.96 & 1.76 & $\mathbf{2.59}$ & $\mathbf{1.25}$ & $\mathbf{4.93}$ & $\mathbf{1.90}$ & $\mathbf{3.07}$ & $\mathbf{1.76}$ & $\mathbf{3.94}$ & $\mathbf{1.72}$ & $\mathbf{3.47}$ & $\mathbf{1.75}$\\
				\hline
				\hline
			\end{tabular}
		\end{center}
	
		%\begin{tablenotes}
		%	\footnotesize
		%	\item $t_{rel}: $ average translational RMSE drift (\%) on length from 100, 200 to 800 m.
		%	\item $r_{rel}: $ average rotational RMSE drift (${}^{\circ}$/100m) on length from 100, 200 to 800 m.
		%\end{tablenotes}
	\caption{Results on ORB-SLAM2 \cite{mur2017orb-slam2}, VISO2-M \cite{geiger2011stereoscan} and our method on the KITTI dataset.}
	\label{tab:table_kitti_00_10_classic}
\end{table}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}

==> fig_table/table_kitti_00_10_dso.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
%\setlength{\tabcolsep}{3.pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table}[t]
	%\scriptsize
	\footnotesize
	%\small
	\centering
		\begin{center}
			\begin{tabular}{ccccccccccc}
				\hline
				\hline
				& \multicolumn{10}{c}{Method} \\
				% \cline{2-15} 
				Seq & \multicolumn{2}{c}{Ours } & \multicolumn{2}{c}{\makecell{VISO2-M \\ \cite{geiger2011stereoscan}}} & \multicolumn{2}{c}{\makecell{DSO \\ \cite{engel2018dso}}} & \multicolumn{2}{c}{\makecell{ORB-SLAM2 \\ \cite{mur2017orb-slam2}}} & \multicolumn{2}{l}{ \makecell{ORB-SLAM2 \\ (LC) \cite{mur2017orb-slam2}}} \\ 
				%Method & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} &  \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} \\
				& $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$  & $t_{rel}$ & $r_{rel}$ \\
				\hline
				% DeepVO &  \multicolumn{2}{c} {$- \quad -$} &  \multicolumn{2}{c}{$8.49 \quad 6.89$} &  \multicolumn{2}{c}{$7.19 \quad 6.97$} &  \multicolumn{2}{c}{$2.62 \quad 3.61$} &  \multicolumn{2}{c}{$5.42 \quad 5.82$} &  \multicolumn{2}{c}{$3.91 \quad 4.60$} &  \multicolumn{2}{c}{$8.11 \quad 8.83$} \\
				%ORB\_SLAM-S [5] & 0.71 & 0.18 & 0.48 & 0.13 & 0.40 & 0.16 & 0.51 & 0.15 & 0.50 & 0.28 & 0.60 & 0.27 \\
				%ORB\_SLAM \cite{mur2017orb-slam2} & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				%ORB\_SLAM-M [5] & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				%VISO2-S \cite{geiger2011stereoscan} & 3.21 & 3.25 & 2.12 & 2.12 & 1.53 & 1.60 & 1.48 & 1.58 & 1.85 & 1.91 & 1.17 & 1.30 \\
				03 & 3.32 & 2.10 & 8.47 & 8.82 & 17.7 & 0.17 & 2.28 & 0.40 &  2.17 & 0.39  \\
				04 & 2.96 & 1.76 & 4.69 & 4.49 & 0.82 & 0.16 & 1.41 & 0.14 & 1.07 & 0.17 \\
				05 & 2.59 & 1.25 & 19.22 & 17.58 & 72.6 & 0.32 & 13.21 & 0.22 & 1.86 & 0.24  \\
				06 & 4.93 & 1.90  & 7.30 & 6.14 & 42.2 & 0.20 & 18.68 & 0.26 & 4.96 & 0.18  \\
				07 & 3.07 & 1.76  & 23.61 & 19.11 & 48.4 & 0.32 & 10.96 & 0.37 & 1.87 & 0.39 \\
				10 & 3.94 & 1.72  & 41.56 & 32.99 & 24.0 & 0.22 & 3.71 & 0.30 & 3.76 & 0.29 \\
				Avg & 3.47 & 1.75 & 17.48 & 16.52 & 34.29 & 0.23 & 8.38 & 0.28 & 2.62 & 0.28 \\
				%VISO2-M \cite{geiger2011stereoscan}   & 8.47 & 8.82 & 4.69 & 4.49 & 19.22 & 17.58 & 7.30 & 6.14 & 23.61 & 19.11 & 41.56 & 32.99 \\
				%\hline
				%\textbf{RNN\_g} & 11.10 & 6.28 & 11.37 & 3.89 & 9.97 & 3.81 & 24.39 & 9.64 & 15.39 & 4.18 & 15.37 & 6.92 \\
				%$\mathbf{RNN}$ & 6.36 & 3.62 & 5.95 & 2.36 & 5.85 & 2.55 & 14.58 & 4.98 & 5.88 & 2.64 & 7.44 & 3.19 & 5.96 & 6.12\\
				
				%$\mathbf{Ours}$  & $\mathbf{3.32}$ & $\mathbf{2.10}$ & 2.96 & 1.76 & $\mathbf{2.59}$ & $\mathbf{1.25}$ & $\mathbf{4.93}$ & $\mathbf{1.90}$ & $\mathbf{3.07}$ & $\mathbf{1.76}$ & $\mathbf{3.94}$ & $\mathbf{1.72}$ & $\mathbf{3.47}$ & $\mathbf{1.75}$\\
				\hline
				\hline
			\end{tabular}
		\end{center}
	
		%\begin{tablenotes}
		%	\footnotesize
		%	\item $t_{rel}: $ average translational RMSE drift (\%) on length from 100, 200 to 800 m.
		%	\item $r_{rel}: $ average rotational RMSE drift (${}^{\circ}$/100m) on length from 100, 200 to 800 m.
		%\end{tablenotes}
	\caption{Results of VISO2-M \cite{geiger2011stereoscan}, ORB-SLAM2 (with and without loop closure) \cite{mur2017orb-slam2} and our method on the KITTI dataset.}
	\label{tab:table_kitti_00_10_classic}
\end{table}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}

==> fig_table/table_kitti_00_10_dso_trans.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
%\setlength{\tabcolsep}{3.pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table}[t]
	%\scriptsize
	%\footnotesize
	%\small
	\centering
		\begin{center}
			\begin{tabular}{cccccc}
				\hline
				\hline
				& \multicolumn{5}{c}{Method} \\
				% \cline{2-15} 
				Seq & {Ours } & {\makecell{VISO2-M \\ \cite{geiger2011stereoscan}}} & {\makecell{DSO \\ \cite{engel2018dso}}} & {\makecell{ORB-SLAM2 \\ \cite{mur2017orb-slam2}}} & { \makecell{ORB-SLAM2 \\ (LC) \cite{mur2017orb-slam2}}} \\ 
				%Method & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} &  \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} \\
				%& $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$  & $t_{rel}$ & $r_{rel}$ \\
				\hline
				% DeepVO &  \multicolumn{2}{c} {$- \quad -$} &  \multicolumn{2}{c}{$8.49 \quad 6.89$} &  \multicolumn{2}{c}{$7.19 \quad 6.97$} &  \multicolumn{2}{c}{$2.62 \quad 3.61$} &  \multicolumn{2}{c}{$5.42 \quad 5.82$} &  \multicolumn{2}{c}{$3.91 \quad 4.60$} &  \multicolumn{2}{c}{$8.11 \quad 8.83$} \\
				%ORB\_SLAM-S [5] & 0.71 & 0.18 & 0.48 & 0.13 & 0.40 & 0.16 & 0.51 & 0.15 & 0.50 & 0.28 & 0.60 & 0.27 \\
				%ORB\_SLAM \cite{mur2017orb-slam2} & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				%ORB\_SLAM-M [5] & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				%VISO2-S \cite{geiger2011stereoscan} & 3.21 & 3.25 & 2.12 & 2.12 & 1.53 & 1.60 & 1.48 & 1.58 & 1.85 & 1.91 & 1.17 & 1.30 \\
				03 & 3.32  & 8.47 & 17.7  & 2.28  &  2.17   \\
				04 & 2.96  & 4.69  & 0.82 & 1.41  & 1.07  \\
				05 & 2.59 & 19.22 & 72.6 &  13.21  & 1.86   \\
				06 & 4.93   & 7.30  & 42.2 & 18.68  & 4.96  \\
				07 & 3.07   & 23.61  & 48.4  & 10.96  & 1.87 \\
				10 & 3.94  & 41.56  & 24.0  & 3.71 & 3.76 \\
				Avg & 3.47 & 17.48  & 34.29 & 8.38 & 2.62  \\
				%VISO2-M \cite{geiger2011stereoscan}   & 8.47 & 8.82 & 4.69 & 4.49 & 19.22 & 17.58 & 7.30 & 6.14 & 23.61 & 19.11 & 41.56 & 32.99 \\
				%\hline
				%\textbf{RNN\_g} & 11.10 & 6.28 & 11.37 & 3.89 & 9.97 & 3.81 & 24.39 & 9.64 & 15.39 & 4.18 & 15.37 & 6.92 \\
				%$\mathbf{RNN}$ & 6.36 & 3.62 & 5.95 & 2.36 & 5.85 & 2.55 & 14.58 & 4.98 & 5.88 & 2.64 & 7.44 & 3.19 & 5.96 & 6.12\\
				
				%$\mathbf{Ours}$  & $\mathbf{3.32}$ & $\mathbf{2.10}$ & 2.96 & 1.76 & $\mathbf{2.59}$ & $\mathbf{1.25}$ & $\mathbf{4.93}$ & $\mathbf{1.90}$ & $\mathbf{3.07}$ & $\mathbf{1.76}$ & $\mathbf{3.94}$ & $\mathbf{1.72}$ & $\mathbf{3.47}$ & $\mathbf{1.75}$\\
				\hline
				\hline
			\end{tabular}
		\end{center}
	
		%\begin{tablenotes}
		%	\footnotesize
		%	\item $t_{rel}: $ average translational RMSE drift (\%) on length from 100, 200 to 800 m.
		%	\item $r_{rel}: $ average rotational RMSE drift (${}^{\circ}$/100m) on length from 100, 200 to 800 m.
		%\end{tablenotes}
	\caption{Results of VISO2-M \cite{geiger2011stereoscan}, ORB-SLAM2 (with and without loop closure) \cite{mur2017orb-slam2} and our method on the KITTI dataset.}
	\label{tab:table_kitti_00_10_classic}
\end{table}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}

==> fig_table/table_tum1.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
\setlength{\tabcolsep}{3.4pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table*}[t]
	%\small
	\centering
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{c||cccccc|c}
				\hline
				\hline
				Sequence & ORB-SLAM2 \cite{mur2017orb-slam2}  & DSO \cite{engel2018dso} & \makecell{Ours \\ (tracking)} & \makecell{Ours \\  (w/o mem atten)} & \makecell{Ours \\ (w/o feat atten)} & \makecell{Ours} & Texture\\
				\hline
				%fr1/desk & X & 1.431 & 1.431  & 0 & 0 & 0 & str/tex\\
				%fr1/desk2 & X & 1.699  & 1.699 & 0 & 0 & 0 & str/tex\\
				%fr2/360 & $\mathbf{0.011}$ & 0.184  & 0.197  & 0 & 0 & str/tex\\
				%fr2/large\_no\_loop & $\mathbf{0.011}$ & 0.015  & 0.  & 0 & 0 & 0 & str/tex\\
				%fr3/long\_office & 0.059 & X  & 0.  & 0 & 0 & 0 & str/tex\\ 
				%\hline
				fr1/xyz & X & 1.526  & 0.2508  & 0 & 0 & 0.168 & object\\
				fr2/desk & X & 1.526  & 0.1826  & 0 & 0 & 0.168 & object\\
				fr2/360\_hemisphere & X & X  & 0.1577  & 0 & 0 & 0.201 & object\\
				fr2/360\_kidnap & 0.184 & 0.197  & 0.3131  & 0 & 0 & 0.233 & object\\
				fr2/pioneer\_360  & X  & X  & 0.241  & 0 & 0 & 0.109 & str\\
				fr2/pioneer\_slam3  & X & 0.737  & 0.149  & 0 & 0 & 0.085& str\\
				fr2/dishes & 0.070 & 0.133  & 0.1448  & 0 & 0 & 0.077 & object\\
				fr2/large\_cabinet & X & 6.838  & 0.1926  & 0 & 0 & 0.201 & object\\
				fr3/sitting\_static & X & 0.082  & 0.0168  & 0 & 0 & 0.201 & object\\
				%fr3/sitting\_xyz & 0.021 & 0.044  & 0 & 0 & 0 & 0.201 & object\\
				fr3/cabinet & X & 2.531  & 0.1578   & 0 & 0 & 0.186 & object\\
				fr3/nstr\_ntex\_near\_loop & X & 2.476  & 0.371 & 0 & 0 & 0.098  & X\\ 
				fr3/nstr\_tex\_near\_loop & 0.057 & 0.093  & 0.046  & 0 & 0 & 0.009 & tex\\ 
				fr3/str\_ntex\_far & X & 0.543  & 0.069  & 0 & 0 & 0.054 & str\\ 
				fr3/str\_tex\_far & 0.018 & 0.040  & 0.080  & 0 & 0 & 0.047 & str/tex\\ 

				
				
				\hline
				\hline
			\end{tabular}	
		\end{center}
	\caption{Evaluation on TUM-RGBD dataset \cite{tum12iros}. The values describe the translational RMSE in [m/s]. Results of ORB-SLAM2 \cite{mur2017orb-slam2} and DSO \cite{engel2018dso} are generated from officially released source code with recommended parameters. \textbf{Ours (tracking)} is a network which just contains the tracking component. \textbf{Ours (w/o mem atten)} indicates the model averages the all memories as input without re-weighting memories according previous output. \textbf{Ours (w/o feat atten)} is the model removing the attention on features.}
	\label{table:tum}
\end{table*}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{2cm}

==> fig_table/table_tum_frames.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
\setlength{\tabcolsep}{3.4pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table*}[t]
	%\small
	\centering
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{ccc||cccccc}
				\hline
				\hline
				Sequence & \makecell{Desc. \\ str/tex/abrupt motion}& Frames & \makecell{5 frames}  & \makecell{ 7 frames} & \makecell{9 frames} & \makecell{11 frames}\\
				\hline
				fr2/desk & Y/Y/N & 2965  & 0.183  & 0.164 & 0.159 & 0.153 \\
				%fr2/360\_hemisphere & Y/Y/N & X & X  & 0.158  & 0.154 & 0.170 & 0.231 \\
				fr2/360\_kidnap & Y/Y/N & 1431  & 0.313  & 0.225 & 0.224 & 0.208 \\
				fr2/pioneer\_360  & Y/Y/Y & 1225 & 0.241  & 0.1338 & 0.076 & \textbf{0.056} \\
				fr2/pioneer\_slam3 & Y/Y/Y & 2544 & 0.149  & 0.1065 & 0.085 & \textbf{0.070}\\
				%fr2/dishes & Y/Y/N & \textbf{0.070} & 0.133  & 0.1448  & 0.1210 & 0.088 & 0.081 \\
				fr2/large\_cabinet & Y/N/N & 1011 & 0.193  & 0.193 & 0.177 & \textbf{0.172} \\
				fr3/sitting\_static & Y/Y/N & 707 & 0.017  & 0.018 & 0.017 &\textbf{0.015} \\
				%fr3/sitting\_xyz & 0.021 & 0.044  & 0 & 0 & 0 & 0.201 & object\\
				%fr3/cabinet & Y/N/N & X & 2.531  & 0.1578   & 0.1660 & 0.190 & 0.196 \\
				fr3/nstr\_ntex\_near\_loop & N/N/N & 1125 & 0.371 & 0.195 & 0.157 & \textbf{0.123} \\ 
				fr3/nstr\_tex\_near\_loop & N/Y/N & 1682   & 0.046  & 0.011 & 0.010 & \textbf{0.007} \\ 
				fr3/str\_ntex\_far & Y/N/N & 814 & 0.069  & 0.047 & 0.039 & \textbf{0.035} \\ 
				fr3/str\_tex\_far & Y/Y/N & 938 & 0.080  & 0.049 & 0.046 &0.042 \\ 
				\hline
				\hline
			\end{tabular}	
		\end{center}
	\caption{Evaluation on the TUM-RGBD dataset \cite{tum12iros}. The values describe the translational RMSE in [m/s]. Results of our model with the \textit{Tracking}, \textit{Memory} and \textit{Refining} components on sequence lengths of 5, 7, 9,11.}
	\label{table:tum}
\end{table*}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{2cm}

==> fig_table/table_tum_frames_tracking.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
\setlength{\tabcolsep}{3.4pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table*}[t]
	%\small
	\centering
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{ccc||cccccc}
				\hline
				\hline
				Sequence & \makecell{Desc. \\ str/tex/abrupt motion}& Frames & \makecell{5 frames}  & \makecell{ 7 frames} & \makecell{9 frames} & \makecell{11 frames}\\
				\hline
				fr2/desk & Y/Y/N & 2965  & 0.183  & 0.164 & 0.159 & 0.153 \\
				%fr2/360\_hemisphere & Y/Y/N & X & X  & 0.158  & 0.154 & 0.170 & 0.231 \\
				fr2/360\_kidnap & Y/Y/N & 1431  & 0.313  & 0.225 & 0.224 & 0.208 \\
				fr2/pioneer\_360  & Y/Y/Y & 1225 & 0.241  & 0.1338 & 0.076 & \textbf{0.056} \\
				fr2/pioneer\_slam3 & Y/Y/Y & 2544 & 0.149  & 0.1065 & 0.085 & \textbf{0.070}\\
				%fr2/dishes & Y/Y/N & \textbf{0.070} & 0.133  & 0.1448  & 0.1210 & 0.088 & 0.081 \\
				fr2/large\_cabinet & Y/N/N & 1011 & 0.193  & 0.193 & 0.177 & \textbf{0.172} \\
				fr3/sitting\_static & Y/Y/N & 707 & 0.017  & 0.018 & 0.017 &\textbf{0.015} \\
				%fr3/sitting\_xyz & 0.021 & 0.044  & 0 & 0 & 0 & 0.201 & object\\
				%fr3/cabinet & Y/N/N & X & 2.531  & 0.1578   & 0.1660 & 0.190 & 0.196 \\
				fr3/nstr\_ntex\_near\_loop & N/N/N & 1125 & 0.371 & 0.195 & 0.157 & \textbf{0.123} \\ 
				fr3/nstr\_tex\_near\_loop & N/Y/N & 1682   & 0.046  & 0.011 & 0.010 & \textbf{0.007} \\ 
				fr3/str\_ntex\_far & Y/N/N & 814 & 0.069  & 0.047 & 0.039 & \textbf{0.035} \\ 
				fr3/str\_tex\_far & Y/Y/N & 938 & 0.080  & 0.049 & 0.046 &0.042 \\ 
				\hline
				\hline
			\end{tabular}	
		\end{center}
	\caption{Evaluation on the TUM-RGBD dataset \cite{tum12iros}. The values describe the translational RMSE in [m/s]. Results of our model with the \textit{Tracking}, \textit{Memory} and \textit{Refining} components on sequence lengths of 5, 7, 9,11.}
	\label{table:tum_frames_tracking}
\end{table*}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{2cm}
